Towards aerodynamic surrogate modeling based on $\beta$-variational autoencoders

Surrogate models that combine dimensionality reduction and regression techniques are essential to reduce the need for costly high-fidelity computational fluid dynamics data. New approaches using $\beta$-Variational Autoencoder ($\beta$-VAE) architectures have shown promise in obtaining high-quality low-dimensional representations of high-dimensional flow data while enabling physical interpretation of their latent spaces. We propose a surrogate model based on latent space regression to predict pressure distributions on a transonic wing given the flight conditions: Mach number and angle of attack. The $\beta$-VAE model, enhanced with Principal Component Analysis (PCA), maps high-dimensional data to a low-dimensional latent space, showing a direct correlation with flight conditions. Regularization through $\beta$ requires careful tuning to improve overall performance, while PCA preprocessing helps to construct an effective latent space, improving autoencoder training and performance. Gaussian Process Regression is used to predict latent space variables from flight conditions, showing robust behavior independent of $\beta$, and the decoder reconstructs the high-dimensional pressure field data. This pipeline provides insight into unexplored flight conditions. Furthermore, a fine-tuning process of the decoder further refines the model, reducing the dependence on $\beta$ and enhancing accuracy. Structured latent space, robust regression performance, and significant improvements in fine-tuning collectively create a highly accurate and efficient surrogate model. Our methodology demonstrates the effectiveness of $\beta$-VAEs for aerodynamic surrogate modeling, offering a rapid, cost-effective, and reliable alternative for aerodynamic data prediction.

==> mainbib <==
@book{fielding2017introduction,
  title={Introduction to aircraft design},
  author={Fielding, J. P.},
  volume={11},
  year={2017},
  publisher={Cambridge University Press}
}

@article{Li2022,
  title = {Machine learning in aerodynamic shape optimization},
  volume = {134},
  ISSN = {0376-0421},
  url = {http://dx.doi.org/10.1016/j.paerosci.2022.100849},
  DOI = {10.1016/j.paerosci.2022.100849},
  journal = {Progress in Aerospace Sciences},
  publisher = {Elsevier BV},
  author = {Li,  Jichao and Du,  Xiaosong and Martins,  Joaquim R.R.A.},
  year = {2022},
  month = oct,
  pages = {100849}
}

@article{yondo2018review,
  title={A review on design of experiments and surrogate models in aircraft real-time and many-query aerodynamic analyses},
  author={Yondo, R. and Andr{\'e}s, E. and Valero, E.},
  journal={Progress in aerospace sciences},
  volume={96},
  pages={23--61},
  year={2018},
  publisher={Elsevier}
}

@article{zhang2021multi,
  title={Multi-fidelity deep neural network surrogate model for aerodynamic shape optimization},
  author={Zhang, X. and Xie, F. and Ji, T. and Zhu, Z. and Zheng, Y.},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={373},
  pages={113485},
  year={2021},
  publisher={Elsevier},
  doi = {10.1016/j.cma.2020.113485}
}

@article{yondo2019review,
  title={A review of surrogate modeling techniques for aerodynamic analysis and optimization: current limitations and future challenges in industry},
  author={Yondo, R. and Bobrowski, K. and Andr{\'e}s, E. and Valero, E.},
  journal={Advances in evolutionary and deterministic methods for design, optimization and control in engineering and sciences},
  doi = {10.1016/j.paerosci.2017.11.003},
  pages={19--33},
  year={2019},
  publisher={Springer}
}

@book{forrester2008engineering,
  title={Engineering design via surrogate modelling: a practical guide},
  author={Forrester, A. and Sobester, A. and Keane, A.},
  year={2008},
  publisher={John Wiley \& Sons}
}

@article{du2021rapid,
  title={Rapid airfoil design optimization via neural networks-based parameterization and surrogate modeling},
  author={Du, X. and He, P. and Martins, J. R.R.A.},
  journal={Aerospace Science and Technology},
  volume={113},
  pages={106701},
  year={2021},
  publisher={Elsevier},
  doi = {10.1016/j.ast.2021.106701},
}

@article{du2022airfoil,
  title={Airfoil design and surrogate modeling for performance prediction based on deep learning method},
  author={Du, Q. and Liu, T. and Yang, L. and Li, L. and Zhang, D. and Xie, Y.},
  journal={Physics of Fluids},
  volume={34},
  number={1},
  year={2022},
  publisher={AIP Publishing},
  DOI = {10.1063/5.0075784},
}

@Article{Wang2019knn,
    AUTHOR = {Wang, L. and Misra, G. and Bai, X.},
    TITLE = {A K Nearest Neighborhood-Based Wind Estimation for Rotary-Wing VTOL UAVs},
    JOURNAL = {Drones},
    VOLUME = {3},
    YEAR = {2019},
    NUMBER = {2},
    ARTICLE-NUMBER = {31},
    ISSN = {2504-446X},
    DOI = {10.3390/drones3020031}
}

@inproceedings{NietoCentenero2023fusing,
  title={Fusing aerodynamic data using multi-fidelity Gaussian process regression},
  series = {EUROGEN 2023},
  booktitle = {15th International Conference on Evolutionary and Deterministic Methods for Design,  Optimization and Control},
  publisher = {Institute of Structural Analysis and Antiseismic Research National Technical University of Athens},
  author = {Nieto-Centenero,  J. and Castellanos,  R. and Gorgues, A. and Andrés,  E.},
  year = {2023},
  collection = {EUROGEN 2023},
  doi = {10.7712/140123.10191.18890}
}

@article{Zhao2022pck,
    title = {Efficient aerodynamic analysis and optimization under uncertainty using multi-fidelity polynomial chaos-Kriging surrogate model},
    journal = {Computers \& Fluids},
    volume = {246},
    pages = {105643},
    year = {2022},
    issn = {0045-7930},
    doi = {10.1016/j.compfluid.2022.105643},
    author = {H. Zhao and Z.-H. Gao and L. Xia}
}

@article{Immordino2024dnn,
    author = {Immordino, G. and Da Ronch, A. and Righi, M.},
    title = {Steady-State Transonic Flowfield Prediction via Deep-Learning Framework},
    journal = {AIAA Journal},
    volume = {62},
    number = {5},
    pages = {1915-1931},
    year = {2024},
    doi = {10.2514/1.J063545}
}

@article{berkooz1993proper,
  title={The proper orthogonal decomposition in the analysis of turbulent flows},
  author={Berkooz, G. and Holmes, P. and Lumley, J.L.},
  journal={Annual review of fluid mechanics},
  volume={25},
  number={1},
  pages={539--575},
  year={1993},
  publisher={Annual Reviews 4139 El Camino Way, PO Box 10139, Palo Alto, CA 94303-0139, USA},
  doi={10.1146/annurev.fl.25.010193.002543}
}

@article{Lucia2004pod,
title = {Reduced-order modeling: new approaches for computational physics},
journal = {Progress in Aerospace Sciences},
volume = {40},
number = {1},
pages = {51-117},
year = {2004},
issn = {0376-0421},
doi = {10.1016/j.paerosci.2003.12.001},
author = {D. J. Lucia and P. S. Beran and W. A. Silva}
}

@article{zimmermann2012pod_cfd, 
    title={Improved extrapolation of steady turbulent aerodynamics using a non-linear POD-based reduced order model}, 
    volume={116}, 
    DOI={10.1017/S0001924000007491}, 
    number={1184}, 
    journal={The Aeronautical Journal (1968)}, 
    publisher={Cambridge University Press}, 
    author={Zimmermann, R. and G\"ortz, S.}, 
    year={2012}, 
    pages={1079–1100}
}

@article{Ly2001PODI,
    title = {Modeling and control of physical processes using proper orthogonal decomposition},
    journal = {Mathematical and Computer Modelling},
    volume = {33},
    number = {1},
    pages = {223-236},
    year = {2001},
    note = {Computation and control VI proceedings of the sixth Bozeman conference},
    issn = {0895-7177},
    doi = {10.1016/S0895-7177(00)00240-5},
    author = {H. V. Ly and H. T. Tran}
}

@article{Bui2004pod,
    author = {Bui-Thanh, T. and Damodaran, M. and Willcox, K.},
    title = {{Aerodynamic Data Reconstruction and Inverse Design Using Proper Orthogonal Decomposition}},
    journal = {AIAA Journal},
    volume = {42},
    number = {8},
    pages = {1505-1516},
    year = {2004},
    doi = {10.2514/1.2159}
}

@article{iuliano2013proper,
  title={Proper orthogonal decomposition, surrogate modelling and evolutionary optimization in aerodynamic design},
  author={Iuliano, E. and Quagliarella, D.},
  journal={Computers \& Fluids},
  volume={84},
  pages={327--350},
  year={2013},
  publisher={Elsevier},
  doi = {10.1016/j.compfluid.2013.06.007},
}

@article{dolci2016proper,
  title={Proper orthogonal decomposition as surrogate model for aerodynamic optimization},
  author={Dolci, V. and Arina, R.},
  journal={International Journal of Aerospace Engineering},
  volume={2016},
  number={1},
  pages={8092824},
  year={2016},
  publisher={Wiley Online Library},
  doi = {10.1155/2016/8092824},
}

@article{dupuis2018surrogate,
  title={Surrogate modeling of aerodynamic simulations for multiple operating conditions using machine learning},
  author={Dupuis, R. and Jouhaud, J.-C. and Sagaut, P.},
  journal={Aiaa Journal},
  volume={56},
  number={9},
  pages={3622--3635},
  year={2018},
  publisher={American Institute of Aeronautics and Astronautics}
}

@article{meilua2024manifold,
  title={Manifold learning: What, how, and why},
  author={Meil{\u{a}}, M. and Zhang, H.},
  journal={Annual Review of Statistics and Its Application},
  volume={11},
  year={2024},
  publisher={Annual Reviews},
  doi={10.1146/annurev-statistics-040522-115238}
}

@article{franz2014interpolation,
  title={Interpolation-based reduced-order modelling for steady transonic flows via manifold learning},
  author={Franz, T. and Zimmermann, R. and G{\"o}rtz, S. and Karcher, N.},
  journal={International Journal of Computational Fluid Dynamics},
  volume={28},
  number={3-4},
  pages={106--121},
  year={2014},
  publisher={Taylor \& Francis},
 doi = {10.1080/10618562.2014.918695}
}

@article{castellanos2022assessment,
  title={An assessment of reduced-order and machine learning models for steady transonic flow prediction on wings},
  author={Castellanos, R. and {Bowen Varela}, J. and Gorgues, A. and Andr{\'e}s, E.},
  journal={ICAS 2022},
  year={2022}
}

@article{halder2024adaptive,
  title={An adaptive sampling algorithm for reduced-order models using Isomap},
  author={Halder, R. and Fidkowski, K.J. and Maki, K.J.},
  journal={International Journal for Numerical Methods in Engineering},
  volume={125},
  number={8},
  pages={e7427},
  year={2024},
  publisher={Wiley Online Library},
  doi = {10.1002/nme.7427}
}

@inproceedings{NietoCentenero2024lle,
    title={Multifidelity surrogate model for efficient aerodynamic predictions},
    author = {Nieto-Centenero,  J. and Mart\'inez-Cava, A. and Andrés,  E.},
    booktitle ={8th European Congress on Computational Methods in Applied Sciences and Engineering},
    year = {2024},
    series = {ECCOMAS Congress 2024},
}

@inproceedings{Castellanos2023isomap,
  series = {EUROGEN 2023},
  title = {Towards aerodynamic shape optimisation by manifold learning and neural networks},
  booktitle = {15th International Conference on Evolutionary and Deterministic Methods for Design,  Optimization and Control},
  publisher = {Institute of Structural Analysis and Antiseismic Research National Technical University of Athens},
  author = {Castellanos,  R. and Nieto-Centenero,  J. and Gorgues,  A. and Discetti,  S. and Ianiro,  A. and Andrés,  E.},
  year = {2023},
  collection = {EUROGEN 2023},
  doi = {10.7712/140123.10190.18887}
}

@article{Carlberg2013GNAT,
    title = {The GNAT method for nonlinear model reduction: Effective implementation and application to computational fluid dynamics and turbulent flows},
    journal = {Journal of Computational Physics},
    volume = {242},
    pages = {623-647},
    year = {2013},
    issn = {0021-9991},
    doi = {10.1016/j.jcp.2013.02.028},
    author = {K. Carlberg and C. Farhat and J. Cortial and D. Amsallem}
}

@article{Chaturantabut2010DEI,
    author = {Chaturantabut, S. and Sorensen, D. C.},
    title = {Nonlinear Model Reduction via Discrete Empirical Interpolation},
    journal = {SIAM Journal on Scientific Computing},
    volume = {32},
    number = {5},
    pages = {2737-2764},
    year = {2010},
    doi = {10.1137/090766498}
}

@article{liao2021multi,
  title={Multi-fidelity convolutional neural network surrogate model for aerodynamic optimization based on transfer learning},
  author={Liao, P. and Song, W. and Du, P. and Zhao, H.},
  journal={Physics of Fluids},
  volume={33},
  number={12},
  year={2021},
  publisher={AIP Publishing}
}

@article{duru2022deep,
  title={A deep learning approach for the transonic flow field predictions around airfoils},
  author={Duru, C. and Alemdar, H. and Baran, O. U.},
  journal={Computers \& Fluids},
  volume={236},
  pages={105312},
  year={2022},
  publisher={Elsevier}
}

@article{deng2023prediction,
  title={Prediction of transonic flow over supercritical airfoils using geometric-encoding and deep-learning strategies},
  author={Deng, Z. and Wang, J. and Liu, H. and Xie, H. and Li, B. and Zhang, M. and Jia, T. and Zhang, Y. and Wang, Z. and Dong, B.},
  journal={Physics of Fluids},
  volume={35},
  number={7},
  year={2023},
  publisher={AIP Publishing}
}

@article{wang2023general,
  title={A general deep transfer learning framework for predicting the flow field of airfoils with small data},
  author={Wang, Z. and Liu, X. and Yu, J. and Wu, H. and Lyu, H.},
  journal={Computers \& Fluids},
  volume={251},
  pages={105738},
  year={2023},
  publisher={Elsevier}
}
@inproceedings{Hines2023mlp,
            year = {2023},
           title = {Physics-based Regularization of Neural Networks for Aerodynamic Flow Prediction},
           pages = {22--39},
          author = {Hines, D. and {Dias Ribeiro}, M. and Bekemeyer, P.},
       booktitle = {EUROGEN 2023  15th ECCOMAS Thematic Conference on  Evolutionary and Deterministic Methods for Design, Optimization and Control},
}

@article{Hines2023gnn,
    title = {Graph neural networks for the prediction of aircraft surface pressure distributions},
    journal = {Aerospace Science and Technology},
    volume = {137},
    pages = {108268},
    year = {2023},
    issn = {1270-9638},
    doi = {10.1016/j.ast.2023.108268},
    author = {D. Hines and P. Bekemeyer}
}

@article{wang2021flow,
  title={Flow field prediction of supercritical airfoils via variational autoencoder based deep learning framework},
  author={Wang, J. and He, C. and Li, R. and Chen, H. and Zhai, C. and Zhang, M.},
  journal={Physics of Fluids},
  volume={33},
  number={8},
  year={2021},
  publisher={AIP Publishing}
}

@article{kang2022physics,
  title={Physics-aware reduced-order modeling of transonic flow via $\beta$-variational autoencoder},
  author={Kang, Y.-E. and Yang, S. and Yee, K.},
  journal={Physics of Fluids},
  volume={34},
  number={7},
  pages={076103},
  year={2022},
  publisher={AIP Publishing LLC},
  doi = {10.1063/5.0097740}
}

@article{wang2023physics,
  title={Physics-assisted reduced-order modeling for identifying dominant features of transonic buffet},
  author={Wang, J. and Xie, H. and Zhang, M. and Xu, H.},
  journal={Physics of Fluids},
  volume={35},
  number={6},
  year={2023},
  publisher={AIP Publishing}
}

@article{beiki2023novel,
  title={Novel attention-based convolutional autoencoder and ConvLSTM for reduced-order modeling in fluid mechanics with time derivative architecture},
  author={Beiki, A. and Kamali, R.},
  journal={Physica D: Nonlinear Phenomena},
  volume={454},
  pages={133857},
  year={2023},
  publisher={Elsevier}
}

@article{kingma2013auto,
  title={Auto-encoding variational bayes},
  author={Kingma, D. P. and Welling, M.},
  journal={arXiv preprint arXiv:1312.6114},
  year={2013},
  doi = {10.48550/ARXIV.1312.6114},
}

@article{eivazi2020deep,
  title={Deep neural networks for nonlinear model order reduction of unsteady flows},
  author={Eivazi, H. and Veisi, H. and Naderi, M. Hossein and Esfahanian, V.},
  journal={Physics of Fluids},
  volume={32},
  number={10},
  pages={105104},
  year={2020},
  publisher={AIP Publishing LLC}
}

@article{zhang2023nonlinear,
  title={Nonlinear mode decomposition via physics-assimilated convolutional autoencoder for unsteady flows over an airfoil},
  author={Zhang, B.},
  journal={Physics of Fluids},
  volume={35},
  number={9},
  year={2023},
  publisher={AIP Publishing}
}

@inproceedings{higgins2017betavae,
  title={$\beta$-vae: Learning basic visual concepts with a constrained variational framework},
  author={Higgins, I. and Matthey, L. and Pal, A. and Burgess, C. and Glorot, X. and Botvinick, M. and Mohamed, S. and Lerchner, A.},
  booktitle={International conference on learning representations},
  year={2017}
}

@article{burgess2018understanding,
  title={Understanding disentangling in $\beta$-{VAE}},
  author={Burgess, C. P. and Higgins, I. and Pal, A. and Matthey, L. and Watters, N. and Desjardins, G. and Lerchner, A.},
  journal={arXiv preprint arXiv:1804.03599},
  year={2018}
}

@article{eivazi2022vae,
  title={Towards extraction of orthogonal and parsimonious non-linear modes from turbulent flows},
  author={Eivazi, H. and Le Clainche, S. and Hoyas, S. and Vinuesa, R.},
  journal={Expert Systems with Applications},
  volume={202},
  pages={117038},
  year={2022},
  publisher={Elsevier}
}

@article{solera2024beta,
  title={$\beta$-Variational autoencoders and transformers for reduced-order modelling of fluid flows},
  author={Solera-Rico, A. and {Sanmiguel Vila}, C. and G{\'o}mez-L{\'o}pez, M. and Wang, Y. and Almashjary, A. and Dawson, S.T.M. and Vinuesa, R.},
  journal={Nature Communications},
  volume={15},
  number={1},
  pages={1361},
  year={2024},
  publisher={Nature Publishing Group UK London}
}

@article{wang2024towards,
  title={Towards optimal $\beta$-variational autoencoders combined with transformers for reduced-order modelling of turbulent flows},
  author={Wang, Y. and Solera-Rico, A. and {Sanmiguel Vila}, C. and Vinuesa, R.},
  journal={International Journal of Heat and Fluid Flow},
  volume={105},
  pages={109254},
  year={2024},
  publisher={Elsevier}
}

@article{Massegur2024gcae,
    doi = {10.1088/2632-2153/ad36ad},
    year = {2024},
    month = {apr},
    publisher = {IOP Publishing},
    volume = {5},
    number = {2},
    pages = {025006},
    author = {D. Massegur and A. {Da Ronch}},
    title = {Graph convolutional multi-mesh autoencoder for steady transonic aircraft aerodynamics},
    journal = {Machine Learning: Science and Technology}
}

@misc{immordino2024gcae,
      title={Predicting Transonic Flowfields in Non-Homogeneous Unstructured Grids Using Autoencoder Graph Convolutional Networks}, 
      author={G. Immordino and A. Vaiuso and A. {Da Ronch} and M. Righi},
      year={2024},
      eprint={2405.04396},
      archivePrefix={arXiv},
      primaryClass={cs.CE}
}

@article{kou2023aeroacoustic,
title = {Aeroacoustic airfoil shape optimization enhanced by autoencoders},
journal = {Expert Systems with Applications},
volume = {217},
pages = {119513},
year = {2023},
doi = {https://doi.org/10.1016/j.eswa.2023.119513},
author = {Kou, J. and Botero-Bolívar, L. and Ballano, R. and Marino, O. and de Santana, L. and Valero, E. and Ferrer, E.},
}

@ARTICLE{Gupta2022dlrom,
  title     = {Three-dimensional deep learning-based reduced order model for
               unsteady flow dynamics with variable Reynolds number},
  author    = {Gupta, R. and Jaiman, R.},
  journal   = {Physics of Fluids},
  volume    =  34,
  number    =  3,
  month     =  mar,
  year      =  2022,
  doi = {https://doi.org/10.1063/5.0082741}
}

@article{moni2024deimvae,
    author = {Moni, Abhijith and Yao, Weigang and Malekmohamadi, Hossein},
    title = "{Data-driven reduced-order modeling for nonlinear aerodynamics using an autoencoder neural network}",
    journal = {Physics of Fluids},
    volume = {36},
    number = {1},
    pages = {016105},
    year = {2024},
    month = {01},
    issn = {1070-6631},
    doi = {10.1063/5.0177577},
    url = {https://doi.org/10.1063/5.0177577}
}

@inproceedings{Pattinson2013xrf1,
  series = {Paper 15A},
  title = {High Fidelity Simulation of the Active Winglet},
  booktitle = {International Forum on Aeroelasticity and Structural Dynamics (IFASD)},
  author = {J. Pattinson and M. Herring},
  year = {2013},
  collection = {EUROGEN 2023},
}

@inbook{Kroll2014tau,
    author = {N. Kroll and S. Langer and A. Schw\"oppe},
    title = {The DLR Flow Solver TAU - Status and Recent Algorithmic Developments},
    booktitle = {52nd Aerospace Sciences Meeting},
    publisher = {American Institute of Aeronautics and Astronautics},
    year={2014},
    doi = {10.2514/6.2014-0080}
}

@article{KullbackLeibler,
 title = {On Information and Sufficiency},
 author = {S. Kullback and R. A. Leibler},
 ISSN = {00034851},
 journal = {The Annals of Mathematical Statistics},
 number = {1},
 pages = {79--86},
 publisher = {Institute of Mathematical Statistics},
 volume = {22},
 year = {1951}
}

@book{williams2006gaussian,
    author = {Rasmussen, C. E. and Williams, C. K. I.},
    title = "{Gaussian Processes for Machine Learning}",
    publisher = {The MIT Press},
    year = {2005},
    month = {11},
    isbn = {9780262256834},
    doi = {10.7551/mitpress/3206.001.0001}
}

@book{gramacy2020surrogates,
  title={Surrogates: Gaussian process modeling, design, and optimization for the applied sciences},
  author={Gramacy, R. B.},
  year={2020},
  publisher={Chapman and Hall/CRC},
  doi = {10.1201/9780367815493},
}

@article{melo2012gaussian,
  title={Gaussian processes for regression: a tutorial},
  author={Melo, J.},
  journal={Technical Report},
  year={2012},
  publisher={University of Porto}
}

@article{Lee2023podvae,
  title = {Parametric model order reduction by machine learning for fluid–structure interaction analysis},
  volume = {40},
  DOI = {10.1007/s00366-023-01782-2},
  number = {1},
  journal = {Engineering with Computers},
  publisher = {Springer Science and Business Media LLC},
  author = {Lee, S. and Jang, K. and Lee, S. and Cho, H. and Shin, S.},
  year = {2023},
  pages = {45–60}
}

@article{Pearson1901pca,
    author = {K. Pearson},
    title = {LIII. On lines and planes of closest fit to systems of points in space },
    journal = {The London, Edinburgh, and Dublin Philosophical Magazine and Journal of Science},
    volume = {2},
    number = {11},
    pages = {559--572},
    year = {1901},
    publisher = {Taylor \& Francis},
    doi = {10.1080/14786440109462720}
}

@article{cantero2023data,
  title={A data-driven approach to suppress artefacts using PCA and autoencoders},
  author={Cantero-Chinchilla, S. and Croxford, A.J. and Wilcox, P.D.},
  journal={NDT \& E International},
  volume={139},
  pages={102904},
  year={2023},
  publisher={Elsevier}
}
